Exploring the Space of Black-box Attacks on Deep Neural Networks

Existing black-box attacks on deep neural networks (DNNs) so far have largely focused on transferability, where an adversarial instance generated for a locally trained model can "transfer" to attack other learning models. In this paper, we propose novel Gradient Estimation black-box attacks for adversaries with query access to the target model's class probabilities, which do not rely on transferability. We also propose strategies to decouple the number of queries required to generate each adversarial sample from the dimensionality of the input. An iterative variant of our attack achieves close to 100% adversarial success rates for both targeted and untargeted attacks on DNNs. We carry out extensive experiments for a thorough comparative evaluation of black-box attacks and show that the proposed Gradient Estimation attacks outperform all transferability based black-box attacks we tested on both MNIST and CIFAR-10 datasets, achieving adversarial success rates similar to well known, state-of-the-art white-box attacks. We also apply the Gradient Estimation attacks successfully against a real-world Content Moderation classifier hosted by Clarifai. Furthermore, we evaluate black-box attacks against state-of-the-art defenses. We show that the Gradient Estimation attacks are very effective even against these defenses.

==> evaluation.tex <==
% In this section, we compare the black-box attacks described in our taxonomy in Section~\ref{sec: taxonomy} through systematic empirical evaluation.
The empirical evaluations carried out on this section are on state-of-the-art neural networks with no defenses.
We consider the attacks outlined in Table~\ref{tab: attack_summary}.
We use two different loss functions in our evaluations, the standard cross-entropy loss (abbreviated as \textgm{xent}) and the logit-based loss (ref. Section~\ref{subsec: logit_loss}) (abbreviated as \textgm{logit}).
All the abbreviations in Table~\ref{tab: attack_summary} denote the untargeted versions of attacks, and the addition of a \textgm{-T} at the end of an abbreviation will denote the targeted version.
In all of these attacks, the adversary's perturbation is constrained using the $L_{\infty}$ distance. Appendix~\ref{subsec: attacks_list} describes these attacks in more detail. Since we find our attacks to closely match white-box attack success, we omit quantitative comparisons with~\cite{papernot2017practical} and~\cite{narodytska2016simple} for lack of space.

\subsection{Evaluation setup for MNIST and CIFAR-10} 
The details of each dataset can be found in Appendix~\ref{subsec: datasets}. The architecture and training details for all models are given in Appendix~\ref{subsec: model_training}.
\noindent \textbf{MNIST} Each pixel of the MNIST image data is scaled to [0,1]. We trained four different models on the MNIST dataset, denoted \textgm{Models A} to \textgm{D}, which are used by Tram\`{e}r et al~\cite{tramer2017ensemble} and represent an interesting variety of architectures. For the attacks constrained with the $L_{\infty}$ distance, we vary the adversary's perturbation budget $\epsilon$ from 0 to 0.4, since at a perturbation budget of 0.5, any image can be made solid gray.
\noindent \textbf{CIFAR-10} Each pixel of the CIFAR-10 image data is in [0,255]. We choose 3 model architectures for this dataset, which we denote as \textsf{Resnet-32}, \textsf{Resnet-28-10} (ResNet variants~\cite{he2016deep,zagoruyko2016wide}) and \textsf{Std-CNN} (a standard CNN~\cite{stdcnnmodel}). For the attacks constrained with the $L_{\infty}$ distance, we vary the adversary's perturbation budget $\epsilon$ from 0 to 28.

\subsection{Metrics}
Throughout this section, we use standard metrics to characterize the effectiveness of various attack strategies. For \emph{MNIST}, all metrics for single-step attacks are computed with respect to the \emph{test set} consisting of 10,000 samples, while metrics for iterative attacks are computed with respect to the first 1,000 samples from the test set. For the \emph{CIFAR-10} data, we choose 1,000 random samples from the test set for single-step attacks and a 100 random samples for iterative attacks.
In our evaluations of targeted attacks, we choose target $T$ for each sample uniformly at random from the set of classification outputs, except the true class $y$ of that sample.

\noindent \textbf{Adversarial success rate.}
% The main metric we will use to measure the effectiveness of an attack will be the adversarial success rate. This represents the fraction of data used that meets the adversary's goal.
The main metric, the adversarial success rate, is the fraction of samples that meets the adversary's goal:
$f(\xad) \neq y$ for untargeted attacks and $f(\xad)=T$ for targeted attacks with target $T$ (\cite{szegedy2014intriguing,tramer2017ensemble}).
% For untargeted attacks, this is the fraction of inputs for which $f(\xad) \neq y$, which is the metric used in most previous work~\cite{szegedy2014intriguing,tramer2017ensemble}. For targeted attacks, it is the fraction of inputs for which $f(\xad)=T$, where $T$ is the target class.
Alternative evaluation metrics are discussed in Appendix~\ref{subsec: alt_metric}.  

\noindent \textbf{Average distortion.}
Another important metric is how much the attack distorts the images, within the budget.
We measure the average $L_2$ distance between the benign samples and the adversarial ones:
\begin{equation}\label{eq: distortion}
    \Delta(\Xad,\bfX) = \frac{1}{N} \sum_{i=1}^N \|(\Xad)_i - (\bfX)_i\|_2
\end{equation}
where $N$ is the number of samples.
This metric allows us to compare the average distortion for attacks which achieve similar adversarial success rates, and therefore infer which one is stealthier.

\noindent \textbf{Number of queries.} Query based black-box attacks make queries to the target model and
this metric may affect the cost of mounting the attack. This is an important consideration when attacking real-world systems which have costs associated with the number of queries made.




\subsection{Summary of Evaluation results}


We first provide a brief summary of the results for both datasets and then describe in further detail the results obtained using each black-box attack. All results for white-box attacks used for comparison are in Appendix~\ref{subsec: whitebox_attacks}.

\noindent\textbf{\fdlogit and \ifdlogit match white-box attack adversarial success rates}:
The \gradientestimation attack with Finite Differences (\fdlogit) is the most successful \emph{untargeted} single-step black-box attack for MNIST and CIFAR-10 models.
It significantly outperforms transferability attacks (Table~\ref{tab: untargeted_blackbox}) and closely tracks white-box FGS with a logit loss (\textgm{WB} \fgslogit) on MNIST and CIFAR-10 (Figure~\ref{fig: bb_all}).
% It significantly outperforms attacks based on transferability, as can be seen in Table~\ref{tab: untargeted_blackbox}. Further, the success rate of this attack closely tracks, and largely coincides with \textgm{WB} \fgslogit for \textsf{Model A} on MNIST and \Rthin on CIFAR-10, as can be seen from Figure~\ref{fig: bb_all}.
For adversarial samples generated iteratively, the Iterative \gradientestimation attack with Finite Differences (\ifdlogit) achieves 100\% adversarial success rate across all models on both datasets (Table~\ref{tab: untargeted_blackbox}). The average distortion for both \fdlogit and \ifdlogit closely matches their white-box counterparts, \fgslogit and \ifgslogit as given in Table~\ref{tab: untargeted_whitebox}. 

\noindent\textbf{\textgm{FD-T} and \textgm{IFD-T} achieve the highest adversarial success rates in the targeted setting}: 
For \emph{targeted} black-box attacks, \ifdxentT achieves 100\% adversarial success rates on almost all models as shown by the results in Table~\ref{tab: targeted_blackbox}. While \fdxentT only achieves about 30\% adversarial success rates, this matches the performance of single-step white-box attacks such as \fgsxentT and \fgslogitT (Table~\ref{tab: targeted_whitebox}). The average distortion for samples generated using gradient estimation methods is similar with that of white-box attacks. 

\noindent\textbf{Gradient estimation with query reduction maintains high adversarial success rates}: For both datasets, the \gradientestimation attack with PCA based query reduction (\fdqrpcalogit) is effective, with performance close to that of \fdlogit with $k=100$ for MNIST (Figure~\ref{fig: feature_est_pca}) and $k=400$ for CIFAR-10 (Figure~\ref{fig: feature_est_pca_CIFAR_10}). The Iterative \gradientestimation attacks with PCA based query reduction (\ifdqrpcalogit) achieve close to 100\% success rates for untargeted attacks and above 80\% for targeted attacks on \textsf{Model A} on MNIST and \Rthin on CIFAR-10 (Figure~\ref{fig: pca_iter_all}).
Figure~\ref{fig: pca_iter_all} clearly shows the effectiveness of the gradient estimation attack across models, datasets and adversarial goals. 
% It achieves close to 100\% success rates for untargeted attacks and above 80\% for targeted attacks.

% On the other hand, the \blindsingle has poor performance when samples are transferred to a model with a very different architecture, as in the transfer from Model \textsf{B} to Model \textsf{D} on MNIST and from \Rwide to \cnnstd on CIFAR-10.
\noindent\textbf{Main takeaway}: When query access to the target model is available, our \gradientestimation attacks using both the Finite Difference method and query reduction outperform transferability based black-box attacks, achieving success rates close to that of the corresponding white-box attacks. These proposed attacks also work on DNNs with defenses, as will be discussed further in Section~\ref{sec: defenses}.

%\noindent\textbf{Remarks.}

\subsection{Detailed Analysis of Evaluation Results}
Now, we examine each of the black-box attack strategies in detail and compare their relative effectiveness, as well as their effectiveness when compared to white-box attacks. As expected, the baseline attacks, i.e. Random-perturbation and Difference-of-means,  are not very effective on either dataset although they do display some interesting characteristics. A brief discussion of the evaluation setup and results for these baseline attacks is contained in Appendix~\ref{subsec: baseline_eval}.


\begin{table} % formerly table 8
    \centering
    \addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{c|cccc}\toprule
    & \multicolumn{4}{c}{\textbf{Untargeted Transferability to \textsf{Model A}}} \\ \midrule
    & \multicolumn{2}{c}{\singlestep} & \multicolumn{2}{c}{\iterative} \\
    \textsf{Source} & \fgsxent & \fgslogit & \ifgsxent & \ifgslogit \\ \bottomrule
    B & 66.3 (6.2) & 80.8 (6.3) & 89.8 (4.75) & 88.5 (4.75)  \\
    B,C & 68.1 (6.2) & 89.8 (6.3) & 95.0 (4.8) & 97.1 (4.9)   \\
    B,C,D & 56.0 (6.3) & 88.7 (6.4) & 73.5 (5.3) & 94.4 (5.3)   \\ \bottomrule
    & \multicolumn{4}{c}{\textbf{Targeted Transferability to \textsf{Model A}}} \\ \midrule
    & \multicolumn{2}{c}{\singlestep} & \multicolumn{2}{c}{\iterative} \\
    \textsf{Source} & \textgm{FGS-T (xent)} & \textgm{FGS-T (logit)} & \textgm{IFGS-T (xent)} & \textgm{IFGS-T (logit)} \\ \bottomrule
    B & 18.3 (6.3) & 18.1 (6.3) & 54.5 (4.6) & 46.5 (4.2)   \\
    B,C & 23.0 (6.3) & 23.0 (6.3) & 76.7 (4.8) & 72.3 (4.5)   \\
    B,C,D & 25.2 (6.4) & 25.1 (6.4) & 74.6 (4.9) & 66.1 (4.7)  \\ \bottomrule
    \end{tabular}
    \caption{Adversarial success rates for \textbf{transferability-based attacks} on \textsf{Model A} (MNIST) at $\epsilon=0.3$. Numbers in parentheses beside each entry give the average distortion $\Delta(\bfX,\Xad)$ over the test set. This table compares the effectiveness of using a single local model to generate adversarial examples versus the use of a local ensemble.}
    \label{tab: MNIST_transfer}
    \addtolength{\tabcolsep}{+3pt}
    \vspace{-20pt}
\end{table}

\subsubsection{Transferability of adversarial examples}\label{subsec: adv_transfer}
For the transferability experiments, we choose to transfer from \textgm{Model B} for MNIST dataset and from \Rwide for CIFAR-10 dataset as these models are each similar to at least one of the other models for their respective dataset, and different from one of the others. They are also fairly representative instances of DNNs used in practice.

Adversarial samples generated using single-step methods and transferred from \textsf{Model B} to the other models have higher success rates for untargeted attacks when they are generated using the logit loss as compared to the cross entropy loss as can be seen in Table~\ref{tab: untargeted_blackbox}. For iterative adversarial samples, however, the untargeted attack success rates are roughly the same for both loss functions. As has been observed before, the adversarial success rate for targeted attacks with transferability is much lower than the untargeted case, even when iteratively generated samples are used. For example, the highest targeted transferability rate in Table~\ref{tab: targeted_blackbox} is 54.5\%, compared to 100.0\% achieved by \ifdxentT across models. One attempt to improve the transferability rate is to use an ensemble of local models, instead of a single one. The results for this on the MNIST data are presented in Table~\ref{tab: MNIST_transfer}. In general, both untargeted and targeted transferability increase when an ensemble is used. However, the increase is not monotonic in the number of models used in the ensemble, and we can see that the transferability rate for \ifgsxent samples falls sharply when \textsf{Model D} is added to the ensemble. This may be due to it having a very different architecture as compared to the models, and thus also having very different gradient directions. This highlights one of the pitfalls of transferability, where it is important to use a local surrogate model similar to the target model for achieving high attack success rates. 

% - Untargeted, FG, logit and cross-entropy\\
% - Untargeted, iterative FG, logit and cross-entropy\\
% - Untargeted, optimization based\\
% - Targeted, FG, logit and cross-entropy\\
% - Targeted, iterative FG, logit and cross-entropy\\
% - Targeted, optimization based\\

\subsubsection{Effectiveness of \gradientestimation using Finite Differences}
In this section, we describe the parameter choices we make for our \gradientestimation attacks with Finite Differences and summarize our results.

\noindent \textbf{Parameter choices}: We use $\delta=1.0$ for \fdxent and \ifdxent for both datasets, while using $\delta=0.01$ for \fdlogit and \ifdlogit. We find that a larger value of $\delta$ is needed for \textgm{xent} loss based attacks to work. The reason for this is that the probability values used in the \textgm{xent} loss are not as sensitive to changes as in the \textgm{logit} loss, and thus the gradient cannot be estimated since the function value does not change at all when a single pixel is perturbed. For the Iterative \gradientestimation attacks using Finite Differences, we use $\alpha=0.01$ and $t=40$ for the MNIST results and $\alpha=1.0$ and $t=10$ for CIFAR-10 throughout. The same parameters are used for the Iterative FGS attack results given in Appendix~\ref{subsec: whitebox_attacks}. This translates to 62720 queries for MNIST (40 steps of iteration) and 61440 queries (10 steps of iteration) for CIFAR-10 per sample. We find these choices work well, and keep the running time of the gradient estimation attacks at a manageable level. However, we find that we can achieve similar adversarial success rates with much fewer queries using query reduction methods which we describe in the next section.

\noindent \textbf{Remarks}: For both targeted and untargeted attacks, we find that the Iterative \gradientestimation attack using Finite Differences is a very powerful attack, achieving 100\% adversarial success rates with low distortion. This holds for both datasets MNIST and CIFAR-10, as can be seen in the results in Tables~\ref{tab: untargeted_blackbox} and~\ref{tab: targeted_blackbox}. We far outperform other black-box attacks such as those based on transferability and match white-box attack success rate.
% Due to this, the finite difference attacks exhibit a larger degree of sensitivity with respect to the choice of loss function, as their adversarial success rate is up to 25 percentage points lower than the white-box case for untargeted attacks when using the cross-entropy loss instead of the logit loss. 



\subsubsection{Query reduction for gradient estimation}
Now, we examine attacks with query reduction when the number of queries is reduced using the random grouping of features as well as using the principal components obtained from PCA. We consider the effectiveness of \gradientestimation with PCA based query reduction and the logit loss (\fdqrrglogit) on \textsf{Model A} in Figure~\ref{fig: feature_est_rg}, where $k$ is the number of indices chosen in each iteration of Algorithm~\ref{alg: random_feat}. Thus, as $k$ increases, we expect the effectiveness to decrease as gradients over larger groups of features are averaged. This is the effect we see in Figure~\ref{fig: feature_est_rg}, where the adversarial success rate drops from 93\% to 63\% at $\epsilon=0.3$ as $k$ increases from 1 to 7. Grouping with $k=7$ translates to 112 queries per MNIST image, down from 784. Thus, in order to achieve high adversarial success rates with the random grouping method, larger perturbation magnitudes are needed.

On the other hand, the PCA-based approach \fdqrpcalogit is a much more effective attack, as can be seen in Figure~\ref{fig: feature_est_pca}. Using 100 principal components to estimate the gradient for \textsf{Model A} on MNIST as in Algorithm~\ref{alg: pca_feat}, the adversarial success rate at $\epsilon=0.3$ is 88.09\%, as compared to 92.9\% without any query reduction. Similarly, using 400 principal components for \Rthin on CIFAR-10 (Figure~\ref{fig: feature_est_pca_CIFAR_10}), an adversarial success rate of 66.9\% can be achieved at $\epsilon=8$. At $\epsilon=16$, the adversarial success rate rises to 80.1\%.


We also evaluate the effectiveness of Iterative \gradientestimation attacks with PCA based query reduction (\ifdqrpcalogit). Note that this attack uses $\alpha=0.04$ and $t=10$ for MNIST and $\alpha=1.0$ and $t=10$ for CIFAR-10. \ifdqrpcalogit with $k=400$ (total of 4000 queries per sample) performs well in both the targeted and untargeted attack cases with $\epsilon=0.3$ for MNIST and $\epsilon=8$ for CIFAR-10 (Figure~\ref{fig: pca_iter_all}), achieving close to 100\% success rates for untargeted attacks and in excess of 80\% for targeted attacks.

\noindent\textbf{Remarks.}
Using 100 to 400 queries per sample for single-step attacks and around 4000 queries per sample for iterative attacks, the gradient estimation attacks are much more effective than transferability based methods in both the targeted and untargeted cases. They surpass the \blindensemble in effectiveness for targeted attacks as well. Since their performance is close to that of white-box attacks, they represent the state-of-the-art in black-box attack capabilities.

% Add a bar chart with the targeted and untargeted attack success rates at different values of K for MNIST and CIFAR-10


% \subsubsection{Transferability with dataset reduction (MNIST)}
% - Untargeted, FG \\
% - Targeted, FG \\ 
% - Untargeted, Optimization based \\
% - Targeted, Optimization based \\ 

% \subsubsection{Which classes are easy to target?}
% - Present results for targeted attacks where all the classes are targeted for each sample.



%% this is for the 'black-box attacks against defenses' section, due to floats
\begin{figure*}[!ht]
\centering
\vspace{-8pt}
\subfloat[\textsf{Model A}\textsubscript{\textsf{adv-0.3}} (MNIST)]{\resizebox{0.49\textwidth}{!}{\input{latex_plots/finite_diff_baseline_linf_Model_A_adv.tex}}\label{subfig: modelA_adv_bb}}
\hspace{0mm}
\subfloat[\Rthin\textsubscript{\textsf{adv-8}} (CIFAR-10)]{\resizebox{0.49\textwidth}{!}{\input{latex_plots/finite_diff_baseline_linf_Resnet_32_adv.tex}}\label{subfig: resnet32_adv_bb}}
\caption{\textbf{Effectiveness of various single step black-box attacks against adversarially trained models}. On the MNIST model, \textsf{Model A}\textsubscript{\textsf{adv-0.3}} the attack with the highest performance up till $\epsilon=0.3$ is the \gradientestimation attack using Finite Differences with initially added randomness. Beyond this, the \blindsingle using samples from Model B performs better. On the CIFAR-10 model \Rthin\textsubscript{\textsf{adv-8}}, the best performing attack is the \blindsingle using samples from \Rwide. }
\label{fig: adv_bb_all}
\vspace{-10pt}
\end{figure*}

\subsection{Practical attacks on Clarifai}
Since the only requirement for carrying out the gradient estimation based attacks is query-based access to the target model, there are a number of deployed public systems providing classification as a service that can be used to evaluate our methods. We choose Clarifai~\cite{clarifai} as it has a number of models trained to classify different image datasets, to which black-box access is provided. In particular, it has models used for the detection of Not Safe For Work (NSFW) content, as well as for content moderation. These are important application domains where the presence of adversarial samples presents a real danger, stemming from the ability of an attacker to make multiple queries to the target model through the API and to generate an adversarial sample which will no longer be classified as inappropriate. For example, an adversary could upload violent images, adversarially modified, such that they are marked incorrectly as safe by the model that underlies the classification API.

We demonstrate an attack of this form on the Clarifai NSFW and Content Moderation models using our gradient estimation based attack. An important point to note here is that these attacks are carried out with \emph{no knowledge of the training set or model}, since both are proprietary information. While some information about the model can be gleaned from news and reports about the website, there is no way to access the training data. In the case of the NSFW and Content Moderation models, this is a crucial advantage that our attack method has over previous techniques, given the lack of an easily accessible open-source dataset for this task. We note here that due to the nature of the images we experiment with, we show only a few of them here, as the majority may be offensive to readers. The full set of images and their classification can be found at \url{https://sunblaze-ucb.github.io/blackbox-attacks/}.

The Content Moderation model has five categories, `safe', `suggestive', `explicit', `drug' and `gore', while the NSFW model has just two categories, `SFW' and `NSFW.' When the API is queried on an image, it returns the confidence scores associated with each category, with the confidence scores summing to 1, like the set of softmax probabilities as in Section~\ref{sec: grad_est_attack}. We attack the models using the gradient estimation attack, and we use the random grouping technique in order to reduce the number of queries. 

An example of an attack on the Content Moderation API is given in Figure~\ref{fig: drug_image_attack}, where the original image on the left (Figure~\ref{subfig: drugs_small}) is clearly of some kind of drug on a table, with a spoon and a syringe. It is classified as a drug by the Content Moderation model with a confidence score of 0.99. The image on the right (Figure~\ref{subfig: drugs_small_adv_32}) is an adversarial image generated with 192 queries to the Content Moderation API, with an $\ell_{\infty}$ constraint on the perturbation of $\epsilon=32$. While the image can still clearly be classified by a human as being of drugs on a table, the Content Moderation model now classifies it as `safe' with a confidence score of 0.96. 
%\bo{try small epsilon for baselines comparing with the random perturbation}

\noindent\textbf{Remarks.} The proposed \gradientestimation attacks can successfully generate adversarial examples that are misclassified on a real-world system hosted by Clarifai with no knowledge of the training set or model.
